RedditBias: A Real-World Resource for Bias Evaluation and Debiasing of Conversational Language Models

Text representation models are prone to exhibit a range of societal biases, reflecting the non-controlled and biased nature of the underlying pretraining data, which consequently leads to severe ethical issues and even bias amplification. Recent work has predominantly focused on measuring and mitigating bias in pretrained language models. Surprisingly, the landscape of bias measurements and mitigation resources and methods for conversational language models is still very scarce: it is limited to only a few types of bias, artificially constructed resources, and completely ignores the impact that debiasing methods may have on the final performance in dialog tasks, e.g., conversational response generation. In this work, we present RedditBias, the first conversational data set grounded in the actual human conversations from Reddit, allowing for bias measurement and mitigation across four important bias dimensions: gender, race, religion, and queerness. Further, we develop an evaluation framework which simultaneously 1) measures bias on the developed RedditBias resource, and 2) evaluates model capability in dialog tasks after model debiasing. We use the evaluation framework to benchmark the widely used conversational DialoGPT model along with the adaptations of four debiasing methods. Our results indicate that DialoGPT is biased with respect to religious groups and that some debiasing techniques can remove this bias while preserving downstream task performance.

==> 07-rw.tex <==
% resources vs methods
% survey
For comprehensive surveys on bias studies in natural language processing, we refer the reader to~\citep{sun-etal-2019-mitigating,blodgett-etal-2020-language} and focus here on sketching the field concerning~(1) methods and resources for bias evaluation, and~(2) bias mitigation methods.

\paragraph{Bias evaluation.} Resources and bias measures initially targeted static word embedding models: with their famous analogy \emph{``man is to computer programmer as woman is to homemaker"}, \citet{bolukbasi} were the first to draw attention to the issue. Later, \citet{caliskan2017semantics} presented the Word Embedding Association Test (WEAT), which quantifies bias between two sets of target terms towards two sets of attribute terms. Subsequent work focused on extensions for more models and languages~\citep[e.g.,][]{mccurdy2020grammatical,lauscher-glavas-2019-consistently,may-etal-2019-measuring,lauscher-etal-2020-araweat},  analysis of proposed measures~\citep[e.g.,][]{gonen2019lipstick,ethayarajh-etal-2019-understanding}, larger frameworks~\citep{lauscher2020general}, and task-specific bias measures and resources, e.g., for co-reference resolution~\citep{zhao-etal-2018-gender}, for natural language inference~\citep{dev2020measuring}, and for machine translation~\citep{stanovsky-etal-2019-evaluating}. 

In our work, we similarly acknowledge the importance of understanding bias w.r.t. downstream tasks, but focus on dialog systems, for which the landscape of research efforts is surprisingly scarce. Here, some authors have more generally discussed bias in natural language generation (NLG): \citet{yeo2020defining} experimented with gender bias in word embeddings for NLG. \citet{webster2020measuring} proposed Discovery of Correlation (DisCo), a template-based method for gender bias detection, which considers a language model's top-3 highest-ranked predictions for a blank text position. While all these works focus on gender bias only, we focus on multiple bias dimension. Similar to us, \citet{sheng-etal-2019-woman} introduced the notion of a regard towards a demographic, based on which they build a dataset as well as a bias classification model. \citet{nadeem2020stereoset} present StereoSet, a crowdsourced dataset for associative contexts at two levels (intrasentence and intersentence) for four bias dimensions and \citet{nangia-etal-2020-crows} presented CrowS-Pairs, a data set for measuring bias in masked LMs focusing on nine bias types. However, they don't measure task-oriented model performance, which may degrade as a result of the debiasing procedure~\citep{lauscher2020general}.
The three only existing works, which truly focus on dialog, are (i) \citet{lee2019exploring} who explore gender-and race bias in chatbots; (ii) \citet{liu2020does}, who construct a benchmark data set for detecting gender and race bias in dialog, and (iii) \citet{dinan-etal-2020-queens}, who analyse existing dialog data sets for gender bias and, based on this, present LIGHT, a bias evaluation resource with a gender-balanced crowd-sourced extension. 
However, none of these works highlights the importance of understanding the effects of debiasing on the models' dialog capabilities and includes established dialog tasks in their evaluation, and none of the existing three works includes more than two bias types.

% methods
\paragraph{Debiasing.} Similar to research on bias evaluation, bias mitigation research initially focused on static word embedding spaces \citep[e.g.,][\emph{inter alia}]{bolukbasi,dev2019attenuating, karve-etal-2019-conceptor, lauscher2020general} and was extended to cover contextualized word embeddings and more tasks~\citep[e.g.,][\emph{inter alia}]{liang-etal-2020-towards,liang-etal-2020-monolingual, zhao-etal-2018-gender}. Generally, the works can be distingished in (1) data-based debiasing methods~\citep{zhao-etal-2017-gender,zhao-etal-2018-gender hall-maudslay-etal-2019-name}, (2) projection-based methods~\citep{bolukbasi} and (3) loss-based debiasing methods~\citep{lauscher2020general}.

representations~\citep{liang-etal-2020-towards}, and general bias direction debiasing~\citep{lauscher2020general}. In this work, the authors also proposed DebiasNet, a method which we adopt as CDD in our experiments. 
We similarly adopt CDA~\citep{zhao-etal-2018-gender}, a popular method that does not rely on a model architecture and has been shown to work for static~\citep{park-etal-2018-reducing} and contextualized embedding spaces~\citep{webster2020measuring, dinan-etal-2020-queens,hall-maudslay-etal-2019-name}. \citet{webster2020measuring} also demonstrated the effectiveness of dropout regularization for debiasing, while \citet{dinan-etal-2020-queens} further focus gender bias reduction by word replacement-based debiasing and conditioned generation.
\citet{liang-etal-2020-monolingual} reduce gender bias in contextualized language models, using DensRay, a method originally intended for interpreting word embeddings. \citet{qian-etal-2019-reducing} reduce gender bias in an LSTM using a loss function based on HD. We adopt their method for pretrained language models.
\citep{sheng-etal-2019-woman} biases in language generation, notation of a regard, regard classification,dataset 

%Demographics: Gender
%Bias measure: Percentage of Male gendered words
%Fine-tuned on encore-decoder transformer model trained on Reddit %dataset
%Mitigation: 
%Counterfactual Data augmentation -  Duplicate sentences with %gendered words but with gender-swapped.
%Positive data: Add manually gender-swapped data to deal with %grammatical errors with automatic augmentation, Add independent %and interesting female personas.
%Controlled training: Control token indicating Gender of the %sentence is used along with sentence in conditional LM training.
%Evaluation: Human-based: Biased dialogues + Engaging dialogues
%Differences: 
%Focus is on Multiple demographics
%our focus is on Decoder based transformer model - DialoGPT %trained on Reddit conversations
%Bias measure is based on Perplexity difference.
%Incorporated controlled training, but used Biased token as for c%onditional LMing.

In contrast to those preceding works, our efforts combine contributions in four directions: we (1) include multiple bias dimensions in our resource and evaluation study, (2) operate on real-world online conversations, (3) focus on a decoder-based transformer model, and (4) focus on the impact of debiasing on models' performances in dialog-oriented tasks. 



